Hyperbolic Generative Adversarial Network

Recently, Hyperbolic Spaces in the context of Non-Euclidean Deep Learning have gained popularity because of their ability to represent hierarchical data. We propose that it is possible to take advantage of the hierarchical characteristic present in the images by using hyperbolic neural networks in a GAN architecture. In this study, different configurations using fully connected hyperbolic layers in the GAN, CGAN, and WGAN are tested, in what we call the HGAN, HCGAN, and HWGAN, respectively. The results are measured using the Inception Score (IS) and the Fr\'echet Inception Distance (FID) on the MNIST dataset. Depending on the configuration and space curvature, better results are achieved for each proposed hyperbolic versions than their euclidean counterpart.

==> include/jlposter.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% myfig
%
% \myfig - replacement for \figure
% necessary, since in multicol-environment 
% \figure won't work        
%                 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\myfig}[3][0]{
\begin{center}
  \vspace{1.5cm}
  \includegraphics[width=#3\hsize,angle=#1]{#2}
  \nobreak\medskip
\end{center}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% mycaption                
%
% \mycaption - replacement for \caption
% necessary, since in multicol-environment \figure and
% therefore \caption won't work
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcounter{figure}
\setcounter{figure}{1}
\newcommand{\mycaption}[1]{
  \vspace{0.5cm}
  \begin{quote}
    {{\sc Figure} \arabic{figure}: #1}
  \end{quote}
  \vspace{1cm}
  \stepcounter{figure}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Some standard colours
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{camlightblue}{rgb}{0.601 , 0.8, 1}
\definecolor{camdarkblue}{rgb}{0, 0.203, 0.402}
\definecolor{camred}{rgb}{1, 0.203, 0}
\definecolor{camyellow}{rgb}{1, 0.8, 0}
\definecolor{lightblue}{rgb}{0, 0, 0.80}
\definecolor{white}{rgb}{1, 1, 1}
\definecolor{whiteblue}{rgb}{0.80, 0.80, 1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Some look and feel definitions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\columnsep}{0.03\textwidth}
\setlength{\columnseprule}{0.0018\textwidth}
\setlength{\parindent}{0.0cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \mysection - replacement for \section*
% 
% Puts a pretty box around some text
% TODO - any other thoughts for what this box should look like
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{mysection} = [rectangle, 
			draw=none, 
			shade, 
			outer color=camlightblue!30,
			inner color=camlightblue!30,
			text width=0.965\columnwidth,
			text centered,
			rounded corners=20pt,
			minimum height=0.09\columnwidth]

\newcommand{\mysection}[1]
{
\begin{center}
  \begin{tikzpicture}
    \node[mysection] {\sffamily\bfseries\LARGE#1};
  \end{tikzpicture}
\end{center}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Set the font
%
% TODO - Not sure what a canonical choice is - feel free to modify
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\familydefault}{cmss}
\sffamily

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%               Background                     %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\background}[3]{
  %\definecolor{cgradbegin}{#1}
  %\definecolor{cgradend}{#2}
 % \psframe[fillstyle=gradient,gradend=cgradend,
 % gradbegin=cgradbegin,gradmidpoint=#3](0.,0.)(1.\textwidth,-1.\textheight)
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                pcolumn                       %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{pcolumn}[1]{
  \begin{minipage}{#1\textwidth}
  \begin{center}
}{
  \end{center}
  \end{minipage}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                pbox                          %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{lcolor}{rgb}{0, 0, 0.80}
\definecolor{gcolor1}{rgb}{1, 1, 1}
\definecolor{gcolor2}{rgb}{.80, .80, 1}

  % \def\fc{fillcolor}
  % \def\getfc #1=#2\par{\def\ffc{#1} \ifx\ffc\fc #2\fi} 
  % \def\getfillcolor #1,#2\par{\getfc #1\par \getfc #2\par}

 %  \newcommand{\psshadowbox}[2]{%[2][magenta]{
%      \fbox{Input arg: #1}
%      \fbox{#1} 
%      \fbox {\getfillcolor #1\par}
%      \def\col{\getfillcolor #1\par}
 
%      \let\coll=\col
%       \coll
 %     \colorbox{\col}{#2}
%       \mbox
   %   \coloredshadowbox{black}{\coll}{#2}
%   }

\newcommand{\pbox}[4]{
%\psshadowbox[#3]{
%\fbox{
\mbox{
\begin{minipage}[t][#2][t]{#1}
#4
\end{minipage}
}%}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Poster environment
%
% Centres everything and can be used to define the width of the content
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{poster}{
  \begin{center}
  \begin{minipage}[c]{\textwidth}
}{
  \end{minipage}
  \end{center}
}

\def\newarrow{\mbox{\begin{tikzpicture}
             \useasboundingbox{(-3pt,-4.5pt) rectangle (19pt,1pt)};
             \draw[->] (0,-0.07)--(17pt,-0.07);\end{tikzpicture}}}



==> repositry.tex <==
\subsection{Generative Adversarial Network (GAN)}

Generative Adversarial Networks \cite{gan} are an architecture of two networks that participate in an adversarial game during training. One, the Generator, is in charge of producing artificial images from noise input. The other, the Discriminator, is in charge of classifying between real images from the artificially generated ones. Therefore, during training, the generated images are passed to the discriminator input, which in turn, alternates artificial and real images. The roles in the adversarial game are as follows: the Generator $G$ is trying to produce images similar to the real ones in order to fool the Discriminator $D$; on the other hand, the Discriminator is trying to detect whether a particular image is real or artificially generated by $G$.\newline
 In this way, the generator $G(\boldsymbol{z};\theta_g)$ learn the distribution $p_{data}$ of the images $\boldsymbol{x}$ from the noise input $\boldsymbol{z}$, and the discriminator $D(\boldsymbol{x};\theta_d)$ estimates the probability of $\boldsymbol{x}$ being real or artificial. Equation \ref{gan} shows the loss function for the GAN, a minimax game, as proposed by \cite{gan}.


 
%\textcolor{violet}{The Gan architecture consists of two neural networks with an adversarial configuration that is to say the networks compete with each other in an optimization game.}

%\textcolor{violet}{ The networks are the discriminator $G$ and generator $G$, where $\theta_g$ and $\theta_d$ are the parameters of the discriminator and generator respectively, the discriminator determines the probability of the image is real, the generator makes images more and more realistic, in other words,  tries to trick the discriminator.
%The training algorithm, in each iteration, gives noise to a generator to make images, these fake images enter the discriminator with the real ones, to obtain the probabilities of realism. Finally, discriminator learns for down the value of realism in the fake images.}


%\textcolor{cyan}{- The gan consist in two neural networks with adversarial configuration}\\
%\textcolor{cyan}{- The networks are the discriminator $D( \cdot, \theta_{d})$ and generator $G( \cdot, \theta_{g})$ where $\theta_{d}$ y $\theta_{g}$ are the parameters of the discriminator and generator respectively}\\
%\textcolor{cyan}{- Both networks play a game of the optimization since discriminator try to go down loss meanwhile generator go up loss that is a minmax optimization}\\
%\textcolor{cyan}{- In the context of the image, the Generator receive as input noise for make the image as output}\\
%\textcolor{cyan}{- unlike to generator the discriminator take the image and determines the probability of the image is real}\\
%\textcolor{cyan}{- in each iteration of training, the generator use a noise for generating images and this images enter to discriminator for estimate the realism, and another hand to discriminator take real images of the dataset }\\


%\textcolor{blue}{La GAN consiste en dos redes neuronales en disposición adversaria, es decir, que la salida de una es la entrada de la otra, y que se entrenan mediante una disputa de optimizadores. Dichas redes consisten en un discriminador $D( \cdot, \theta_{d})$ y un generador $G( \cdot, \theta_{g})$, donde $\theta_{d}$ y $\theta_{g}$ son los parámetros del discriminador y el generador respectivamente.\newline
%En el contexto de imágenes, el Generador es una red que en su entrada recibe ruido y en su salida pretende generar imágenes similares a las reales o del set de entrenamiento. El discriminador es un red que en su entrada recibe una imagen (puede ser real o generada) y en su salida estima la probabilidad que esa imagen sea real.\newline
%De esta forma en cada iteración del entrenamiento, el generador recibe un ruido $\boldsymbol{z}$, para generar una imagen cuya probabilidad de ser real es estimada por el discriminador $D$, y se realiza un paso de optimización de los parámetros $\theta_{g}$ de acuerdo al funcional de costo $J_g$ de la ecuación \eqref{Jg} \cite{gan}. Luego, el discriminador recibe una imagen real, y en función de la probabilidad asignada tanto a la imagen real como a la generada, se realiza un paso de optimización de los parámetros $\theta_{d}$ de acuerdo al funcional de costo $J_d$ de la ecuación \eqref{Jd} \cite{gan}. En cada iteración estos dos pasos son repetidos, hasta que el entrenamiento finaliza cuando la probabilidad entregada por el discriminador alcanza un valor cercano al $0.5$ para las imágenes generadas, puesto que en este momento el discriminador y generador han alcanzado su óptimo.}


%\begin{equation}\label{Jg}
%    J_{g}(z) = -log(D(G(z;\theta_{g}),\theta_{d}))
%\end{equation}
%\begin{equation}\label{Jd}
%    J_{d}(x_{real}, z) = -log(D(x_{real};\theta_{d}))-log(1-D(G(z;\theta_{g}),\theta_{d}))
%\end{equation}

\begin{equation}\label{gan}
\begin{aligned}
 \min\limits_{G}\max\limits_{D}\; V(D,G) \; = \; & {} \mathbb{E}\limits_{\boldsymbol{x}\sim p_{data}(\boldsymbol{x})}[\log D(\boldsymbol{x})] \\
                                         & {} + \mathbb{E}\limits_{\boldsymbol{z}\sim p_z(\boldsymbol{z})}[\log(1 - D(G(\boldsymbol{z}))]
\end{aligned}
\end{equation}
The training finish when the discriminator is unable to distinguish between real from generated images. Once trained the GAN generator network can be used independently for generating images. However, it is not possible to control the output in any way, as in with the MNIST dataset. The GAN network can also be difficult to train showing vanishing gradients and mode collapse, more details about this issues can be found in \cite{gan_train}. In this work we use two modifications to the original GAN architecture, the  Conditional GAN  (CGAN) \cite{cgan} and the Wasserstein GAN (WGAN) \cite{wgan}. The CGAN includes an additional input layer at both the Generator and Discriminator that allows to condition the generation and classification task. This additional information can be used to specify a class, like a digit ,for example,  when working with the MNIST dataset.  Equation \ref{cgan} shows the loss function for the CGAN which includes the additional information $\boldsymbol{y}$ for conditioning at the Discriminator and Generator.
\begin{equation}\label{cgan}
\begin{aligned}
\min \limits_{G} \max \limits_{D}\; V(D, G) \; = \; & {}\mathbb{E}_{\boldsymbol{x} \sim p_{\text {data }}(\boldsymbol{x})}[\log D(\boldsymbol{x} | \boldsymbol{y})] \\ 
 & {} + \mathbb{E}_{\boldsymbol{z} \sim p_{\boldsymbol{z}}(\boldsymbol{z})}[\log (1-D(G(\boldsymbol{z} | \boldsymbol{y})))]
\end{aligned}
\end{equation}
The WGAN addresses the issues of vanishing gradients and mode collapse of the original GAN architecture. To achieve this goal they use the equation \ref{wgan} where the supremum is all over 1-Lipschitz functions $f$.

\begin{equation}\label{wgan}
W\left(\mathbb{P}_{r}, \mathbb{P}_{\theta}\right)=\sup _{\|f\|_{L} \leq 1} \mathbb{E}_{x \sim \mathbb{P}_{r}}[f(x)]-\mathbb{E}_{x \sim \mathbb{P}_{\theta}}[f(x)]
\end{equation}



\subsection{Hyperbolic Deep Learning}

Deep Neural Networks learn abstract features from the data through their neural layers that sequentially process the data, with more abstract representation in the more profound layers\cite{representation}. The conventional \textcolor{red}{neural networks} \sout{layers} \textcolor{red}{are designed} \sout{have} under the assumption that the data has Euclidean nature or grid-like structure; therefore, the layers have euclidean operations like addition, distance, metric, and multiplication. However, conventional neural networks may not provide the best representation if the data exhibit a non-euclidean nature \textcolor{red}{, like text, riemmanian manifolds, 3D images, graphs, etc. \cite{gdl}}. \textcolor{red}{Data that presents a hierarchical structure, or cyclical structure, are examples where the euclidean representation may not be the best. Cyclical behavior can be represented by spherical spaces (positive curvature), on the other hand hierarchical data can be well represented in an hyperbolic space (negative curvature). Hyperbolic Geometry is appropriate to represent the hierarchy of the data due to the fact that Hyperbolic space has the same metric structure than trees \cite{hyp_geo_comp_net}. The pointcare ball representation of an hyperbolic space let us to represent hierarchical data with less distortion and dimensions than the euclidean space \cite{poincemb}.  To exploit the hierarchical nature of data, Ganea et al. propose a Hyperbolic Neural Network (HNN)\cite{hnn} that consists of Neural Networks that work in the Poincaré Ball model. The HNN does all operations in the Poincaré Ball through the frameworks of gyrovectors space\cite{gyrovector}. It gives equivalent Euclidean algebraic operations in the Hyperbolic spaces.  The HNN improves the task of textual entailment, it also has showed good results in  node classification and link prediction with the use of Hyperbolic Graph Convolutional Neural Network \cite{hgcnn}.\\ 
For images, they can also present hierarchical behavior, like the relationship between hierarchical characteristics in language and images such as ImageNet\cite{imagenet} that is an image database organized according to the WordNet (REFERENCIA!) hierarchy. Khrulkov et al. \cite{hyime} argue the possibility of using HNN to leverage the natural hierarchy in the images. }

\textcolor{red}{AGREGAR NUESTRA PROPUESTA}

\sout{When data present this nature, it has specific structural and geometrical properties}.
\sout{Therefore,} for processing this kind of data, we require \sout{new} layers that leverage the non-Euclidean properties of the data \cite{gdl}. \sout{ Examples of this data with non-Euclidean nature are graph \cite{social_network_data} or images 3d\cite{data_3d}}.

Some of the concepts where Euclidean metrics does not work are the similarity that has cyclic behavior, and the hierarchy has tree behavior \cite{mixcurv}. The cyclic behavior match with Spherical Geometry \cite{spherical_emb} and hierarchy with Hyperbolic geometry \cite{poincemb}. The structural properties depend on the particular space, but in hyperbolic spaces, the critical behavior is the hierarchy. The geometrical properties in general non-euclidean space are characterized by geodesic that not necessary is a straight line and particularly in hyperbolic space by the divergence of the parallels. Hyperbolic Geometry is appropriate to represent the hierarchy of the data due that Hyperbolic space has the same metric structure that trees \cite{hyp_geo_comp_net}. Therefore Hyperbolic spaces like Poincaré Disk are perfect to represent hierarchies with less distortion and dimension that Euclidean Space \cite{poincemb}.\newline
To exploit the hierarchical nature of data Ganea et al. proposes a Hyperbolic Neural Network (HNN)\cite{hnn} that consists of Neural Networks embedded in the Poincaré Disk. The HNN does all operations in the Poincaré Disk through the frameworks of gyrovectors space\cite{gyrovector}. It gives equivalent Euclidean algebraic in the Hyperbolic spaces.  The HNN improves the task of textual entailment, other applications of the HNN are in graphs with Hyperbolic Graph Convolutional Neural Network \cite{hgcnn} that improved the tasks of node classification and link prediction.
\newline
Exist many hierarchical characteristics in the image; an example of this characteristic is the natural relation between hierarchical characteristics in language and images, such as ImageNet \cite{imagenet} that is an image database organized according to the WordNet hierarchy. Khrulkov et al. \cite{hyime} argue the possibility of using HNN to leverage the natural hierarchy in the images. In this work, the authors propose a Hyperbolic Image Embedding, where mix euclidean layers with hyperbolic layers,  furthermore the use of exponential and logarithm map to connect both spaces to improve few-shot classification task. 



==> tables/architecture-comparison.tex <==


\def\layersep{1.5cm}
\def\nodesep{0.500cm}
\def\nodesize{0.36cm}

\newcommand{\numdims}[0]{5}
\newcommand{\numhidden}[0]{5}
\newcommand{\upnodedist}[0]{0.36cm}
\newcommand{\bardist}[0]{\hspace{-0.03cm}}
\begin{figure*}[htb!]
\centering
\begin{tabular}{cc}
\bardist 
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{hyperbolic layer}=[neuron, fill=red!50];
    \tikzstyle{euclidean layer}=[neuron, fill=blue!50];
    \tikzstyle{to poincare}=[neuron, fill=green!50];
    \tikzstyle{from poincare}=[neuron, fill=yellow!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,3}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \path[yshift=-0.6cm]
        node[euclidean layer, minimum size=\nodesize
        %, pin=left:Input \#\y
        ] (I-\name) at (0,-1.2*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=-0.6cm]
            node[euclidean layer, minimum size=\nodesize] (E1-\name) at (0.7*\layersep,-1*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,5}
        \path[yshift=-0.4cm]
            node[euclidean layer, minimum size=\nodesize] (E2-\name) at (1.4*\layersep, -0.95*\nodesep*\y) {};
            
    \foreach \name / \y in {1,...,5}
        \path[yshift=-0.1cm]
            node[to poincare, minimum size=\nodesize] (TP-\name) at (2.1*\layersep,-1.15*\nodesep*\y) {};

    \foreach \name / \y in {1,...,6}
        \path[yshift=0.195cm]
            node[hyperbolic layer, minimum size=\nodesize] (H1-\name) at (2.8*\layersep,-1.1*\nodesep*\y) {};
            
    \foreach \name / \y in {1,...,4}
        \path[yshift=0.05cm]
            node[hyperbolic layer, minimum size=\nodesize] (H2-\name) at (3.5*\layersep,-1.4*\nodesep*\y) {};
    
    \foreach \name / \y in {1,...,4}
        \path[yshift=0.07cm]
            node[from poincare, minimum size=\nodesize] (FP-\name) at (4.2*\layersep,-1.4*\nodesep*\y) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,4}
            \path (I-\source) edge (E1-\dest);
            
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,5}
            \path (E1-\source) edge (E2-\dest);
            
    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,5}
            \path (E2-\source) edge (TP-\dest);
            
    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,6}
            \path (TP-\source) edge (H1-\dest);
            
    \foreach \source in {1,...,6}
        \foreach \dest in {1,...,4}
            \path (H1-\source) edge (H2-\dest);
            
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,4}
            \path (H2-\source) edge (FP-\dest);
    % Annotate the layers
    \node[annot,above of=I-1, node distance=\upnodedist] {Noise};
    \node[annot,above of=E1-1, node distance=\upnodedist] {Euc};
    \node[annot,above of=E2-1, node distance=\upnodedist] {Euc};
    \node[annot,above of=TP-1, node distance=\upnodedist] {TP};
    \node[annot,above of=H1-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=H2-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=FP-1, node distance=\upnodedist] {FP};
\end{tikzpicture}
\bardist
&
\bardist
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{hyperbolic layer}=[neuron, fill=red!50];
    \tikzstyle{euclidean layer}=[neuron, fill=blue!50];
    \tikzstyle{to poincare}=[neuron, fill=green!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[euclidean layer, minimum size=\nodesize
        %, pin=left:Input \#\y
        ] (I-\name) at (0,-1.5*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,7}
        \path[yshift=0.2cm]
            node[euclidean layer, minimum size=\nodesize] (E1-\name) at (0.7*\layersep,-\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,5}
        \path[yshift=0.3cm]
            node[euclidean layer, minimum size=\nodesize] (E2-\name) at (1.4*\layersep,-1.3*\nodesep*\y) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,5}
    	\node[to poincare, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (TP-\name) at (2.1*\layersep,-1.15*\nodesep*\y) {};
    


    % Draw the output layer node
    \foreach \name / \y in {1,...,3}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H1-\name) at (2.8*\layersep,-1.7*\nodesep*\y) {};
    	
    \foreach \name / \y in {1,...,1}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H2-\name) at (3.5*\layersep,-3.4*\nodesep*\y) {};
    	


    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,7}
            \path (I-\source) edge (E1-\dest);
            
    \foreach \source in {1,...,7}
        \foreach \dest in {1,...,5}
            \path (E1-\source) edge (E2-\dest);     
            
    \foreach \source in {1,...,5}
    \foreach \dest in {1,...,5}
    \path (E2-\source) edge (TP-\dest);
            
    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,3}
            \path (TP-\source) edge (H1-\dest);                

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,1}
    	    \path (H1-\source) edge (H2-\dest);

    % Annotate the layers
    \node[annot,above of=I-1, node distance=\upnodedist] {Image};
    \node[annot,above of=E1-1, node distance=\upnodedist] {Euc};
    \node[annot,above of=E2-1, node distance=\upnodedist] {Euc};
    \node[annot,above of=TP-1, node distance=\upnodedist] {TP};
    \node[annot,above of=H1-1, node distance=\upnodedist]{Hyp};
    \node[annot,above of=H2-1, node distance=\upnodedist]{Hyp};

\end{tikzpicture} \\
Generator Network: & 
Discriminator Network:\\ $Gen = FP \circ Hyp \circ Hyp \circ TP \circ Euc \circ Euc $  &$Dis = Hyp \circ Hyp \circ TP \circ Euc \circ Euc $
\end{tabular}
\caption{fefkejk}
\end{figure*}

==> tables/architecture-hgan_dis3.tex <==
\def\layersep{3.33cm}
\def\nodesep{1.25cm}
\def\nodesize{0.8cm}

\newcommand{\numdims}[0]{5}
\newcommand{\numhidden}[0]{5}
\newcommand{\upnodedist}[0]{1.2cm}
\newcommand{\bardist}[0]{\hspace{-0.2cm}}

\begin{tabular}{c}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{hyperbolic layer}=[neuron, fill=red!50];
    \tikzstyle{euclidean layer}=[neuron, fill=blue!50];
    \tikzstyle{to poincare}=[neuron, fill=green!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[euclidean layer, minimum size=\nodesize
        %, pin=left:Input \#\y
        ] (I-\name) at (0,-1.5*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,7}
        \path[yshift=0.5cm]
            node[euclidean layer, minimum size=\nodesize] (E1-\name) at (0.7*\layersep,-\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,7}
        \path[yshift=0.5cm]
            node[to poincare, minimum size=\nodesize] (E2-\name) at (1.4*\layersep,-\nodesep*\y) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,5}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (TP-\name) at (2.1*\layersep,-1.15*\nodesep*\y) {};
    


    % Draw the output layer node
    \foreach \name / \y in {1,...,3}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H1-\name) at (2.8*\layersep,-1.7*\nodesep*\y) {};
    	
    \foreach \name / \y in {1,...,1}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H2-\name) at (3.5*\layersep,-3.4*\nodesep*\y) {};
    	


    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,7}
            \path (I-\source) edge (E1-\dest);
            
    \foreach \source in {1,...,7}
        \foreach \dest in {1,...,7}
            \path (E1-\source) edge (E2-\dest);     
            
    \foreach \source in {1,...,7}
    \foreach \dest in {1,...,5}
    \path (E2-\source) edge (TP-\dest);
            
    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,3}
            \path (TP-\source) edge (H1-\dest);                

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,1}
    	    \path (H1-\source) edge (H2-\dest);

    % Annotate the layers
    \node[annot,above of=I-1, node distance=\upnodedist] {Image};
    \node[annot,above of=E1-1, node distance=\upnodedist] {Euc};
    \node[annot,above of=E2-1, node distance=\upnodedist] {TP};
    \node[annot,above of=TP-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=H1-1, node distance=\upnodedist]{Hyp};
    \node[annot,above of=H2-1, node distance=\upnodedist]{Hyp};
\end{tikzpicture}
\end{tabular}


==> tables/architecture-hgan_dis4.tex <==
\def\layersep{3.33cm}
\def\nodesep{1.25cm}
\def\nodesize{0.8cm}

\newcommand{\numdims}[0]{5}
\newcommand{\numhidden}[0]{5}
\newcommand{\upnodedist}[0]{1.2cm}
\newcommand{\bardist}[0]{\hspace{-0.2cm}}

\begin{tabular}{c}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{hyperbolic layer}=[neuron, fill=red!50];
    \tikzstyle{euclidean layer}=[neuron, fill=blue!50];
    \tikzstyle{to poincare}=[neuron, fill=green!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[euclidean layer, minimum size=\nodesize
        %, pin=left:Input \#\y
        ] (I-\name) at (0,-1.5*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=1.1cm]
            node[to poincare, minimum size=\nodesize] (E1-\name) at (0.7*\layersep,-1.8*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,7}
        \path[yshift=0.5cm]
            node[hyperbolic layer, minimum size=\nodesize] (E2-\name) at (1.4*\layersep,-1*\nodesep*\y) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,5}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (TP-\name) at (2.1*\layersep,-1.15*\nodesep*\y) {};
    


    % Draw the output layer node
    \foreach \name / \y in {1,...,3}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H1-\name) at (2.8*\layersep,-1.7*\nodesep*\y) {};
    	
    \foreach \name / \y in {1,...,1}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H2-\name) at (3.5*\layersep,-3.4*\nodesep*\y) {};
    	


    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,4}
            \path (I-\source) edge (E1-\dest);
            
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,7}
            \path (E1-\source) edge (E2-\dest);     
            
    \foreach \source in {1,...,7}
    \foreach \dest in {1,...,5}
    \path (E2-\source) edge (TP-\dest);
            
    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,3}
            \path (TP-\source) edge (H1-\dest);                

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,1}
    	    \path (H1-\source) edge (H2-\dest);

    % Annotate the layers
    \node[annot,above of=I-1, node distance=\upnodedist] {Image};
    \node[annot,above of=E1-1, node distance=\upnodedist] {TP};
    \node[annot,above of=E2-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=TP-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=H1-1, node distance=\upnodedist]{Hyp};
    \node[annot,above of=H2-1, node distance=\upnodedist]{Hyp};
\end{tikzpicture}
\end{tabular}


==> tables/architecture-toronto.tex <==
\def\layersep{3.33cm}
\def\nodesep{1.25cm}
\def\nodesize{0.8cm}

\newcommand{\numdims}[0]{5}
\newcommand{\numhidden}[0]{5}
\newcommand{\upnodedist}[0]{1.2cm}
\newcommand{\bardist}[0]{\hspace{-0.2cm}}

\begin{tabular}{c|c}
\bardist
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{hyperbolic layer}=[neuron, fill=red!50];
    \tikzstyle{euclidean layer}=[neuron, fill=blue!50];
    \tikzstyle{to poincare}=[neuron, fill=green!50];
    \tikzstyle{from poincare}=[neuron, fill=yellow!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,3}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[euclidean layer, minimum size=\nodesize
        %, pin=left:Input \#\y
        ] (I-\name) at (0,-1.5*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,3}
        \path[yshift=0cm]
            node[to poincare, minimum size=\nodesize] (E1-\name) at (0.7*\layersep,-1.5*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=0.75cm]
            node[hyperbolic layer, minimum size=\nodesize] (E2-\name) at (1.4*\layersep,-1.4*\nodesep*\y) {};
            
    \foreach \name / \y in {1,...,5}
        \path[yshift=1.8cm]
            node[hyperbolic layer, minimum size=\nodesize] (TP-\name) at (2.1*\layersep,-1.4*\nodesep*\y) {};

    \foreach \name / \y in {1,...,6}
        \path[yshift=1.95cm]
            node[hyperbolic layer, minimum size=\nodesize] (H1-\name) at (2.8*\layersep,-1.2*\nodesep*\y) {};
            
    \foreach \name / \y in {1,...,4}
        \path[yshift=1cm]
            node[hyperbolic layer, minimum size=\nodesize] (H2-\name) at (3.5*\layersep,-1.4*\nodesep*\y) {};
    
    \foreach \name / \y in {1,...,4}
        \path[yshift=1cm]
            node[from poincare, minimum size=\nodesize] (FP-\name) at (4.2*\layersep,-1.4*\nodesep*\y) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,3}
            \path (I-\source) edge (E1-\dest);
            
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,4}
            \path (E1-\source) edge (E2-\dest);
            
    \foreach \source in {1,...,4}
    \foreach \dest in {1,...,5}
    \path (E2-\source) edge (TP-\dest);
            
    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,6}
            \path (TP-\source) edge (H1-\dest);
            
    \foreach \source in {1,...,6}
        \foreach \dest in {1,...,4}
            \path (H1-\source) edge (H2-\dest);
            
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,4}
            \path (H2-\source) edge (FP-\dest);
    % Annotate the layers
    \node[annot,above of=I-1, node distance=\upnodedist] {Noise};
    \node[annot,above of=E1-1, node distance=\upnodedist] {TP};
    \node[annot,above of=E2-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=TP-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=H1-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=H2-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=FP-1, node distance=\upnodedist] {FP};
\end{tikzpicture}
\bardist
&
\bardist
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{hyperbolic layer}=[neuron, fill=red!50];
    \tikzstyle{euclidean layer}=[neuron, fill=blue!50];
    \tikzstyle{to poincare}=[neuron, fill=green!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[euclidean layer, minimum size=\nodesize
        %, pin=left:Input \#\y
        ] (I-\name) at (0,-1.5*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=1.1cm]
            node[to poincare, minimum size=\nodesize] (E1-\name) at (0.7*\layersep,-1.8*\nodesep*\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,7}
        \path[yshift=0.5cm]
            node[hyperbolic layer, minimum size=\nodesize] (E2-\name) at (1.4*\layersep,-1*\nodesep*\y) {};

    % Draw the output layer node
    \foreach \name / \y in {1,...,5}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (TP-\name) at (2.1*\layersep,-1.15*\nodesep*\y) {};
    


    % Draw the output layer node
    \foreach \name / \y in {1,...,3}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H1-\name) at (2.8*\layersep,-1.7*\nodesep*\y) {};
    	
    \foreach \name / \y in {1,...,1}
    	\node[hyperbolic layer, minimum size=\nodesize
    	%,pin={[pin edge={->}]right:Output }
    	] (H2-\name) at (3.5*\layersep,-3.4*\nodesep*\y) {};
    	


    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,4}
            \path (I-\source) edge (E1-\dest);
            
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,7}
            \path (E1-\source) edge (E2-\dest);     
            
    \foreach \source in {1,...,7}
    \foreach \dest in {1,...,5}
    \path (E2-\source) edge (TP-\dest);
            
    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,3}
            \path (TP-\source) edge (H1-\dest);                

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,1}
    	    \path (H1-\source) edge (H2-\dest);

    % Annotate the layers
    \node[annot,above of=I-1, node distance=\upnodedist] {Image};
    \node[annot,above of=E1-1, node distance=\upnodedist] {TP};
    \node[annot,above of=E2-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=TP-1, node distance=\upnodedist] {Hyp};
    \node[annot,above of=H1-1, node distance=\upnodedist]{Hyp};
    \node[annot,above of=H2-1, node distance=\upnodedist]{Hyp};
\end{tikzpicture} \\
Generator Network: & 
Discriminator Network:\\ $Gen = FP \circ H \circ H \circ H \circ H \circ TP$  &$Dis = H \circ H \circ H \circ H \circ TP$
\end{tabular}


==> tables/input-connected.tex <==
\def\layersep{4cm}
\def\nodeseptwo{3.5cm}
\def\nodesize{.45cm}

\begin{tabular}{ccc}
\bardist
\begin{tikzpicture}[draw=black!80]
    \tikzstyle{neuron}=[circle,minimum size=17pt, draw = black!80, fill = white, thick]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{pile} =[thick, ->, >=stealth', shorten <=7pt, shorten >=8pt];

    % Define the input layer node
    \coordinate (I) at (0, 0);


    % Define the hidden layer nodes
    \foreach \name / \y in {1,...,\numhidden}
    {
        \coordinate (H-\name) at (\nodeseptwo*\y, 0);
    }

    % Connect every node            
    \foreach \name in {1,...,\numhidden}
    {
	 \path[pile] (I) edge (H-\name) {};
         %\path[pile] (I) edge [bend left] (H-\name) {};
    }

    \draw (I) node[neuron] {};
    \draw (I) node[below = 0.5cm]  {$\vx$};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,\numhidden}
    {
	\draw (H-\name) node[neuron]  {};
        \draw (H-\name) node[below = 0.34cm] {$\vf^{(\y)}(\vx)$};
    }
\end{tikzpicture} & \hspace{2cm} &
\bardist
\begin{tikzpicture}[draw=black!80]
    \tikzstyle{neuron}=[circle,minimum size=17pt, draw = black!80, fill = white, thick]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{pile} =[thick, ->, >=stealth', shorten <=7pt, shorten >=8pt];

    % Define the input layer node
    \coordinate (I) at (0, 0);


    % Define the hidden layer nodes
    \foreach \name / \y in {1,...,\numhidden}
    {
        \coordinate (H-\name) at (\nodeseptwo*\y, 0);
    }

    % Connect every node            
    \foreach \name in {1,...,\numhidden}
    {
	 \path[pile] (I) edge (H-\name) {};
         \path[pile] (I) edge [bend left] (H-\name) {};
    }

    \draw (I) node[neuron] {};
    \draw (I) node[below = 0.5cm]  {$\vx$};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,\numhidden}
    {
	\draw (H-\name) node[neuron]  {};
        \draw (H-\name) node[below = 0.34cm] {$\vf^{(\y)}(\vx)$};
    }
\end{tikzpicture} \\
Standard \MLP{} architecture. & & Input-connected architecture.
\end{tabular}

